Pop Quiz! Do Pre-trained Code Models Possess Knowledge of Correct API Names?

Recent breakthroughs in pre-trained code models, such as CodeBERT and Codex, have shown their superior performance in various downstream tasks. The correctness and unambiguity of API usage among these code models are crucial for achieving desirable program functionalities, requiring them to learn various API fully qualified names structurally and semantically. Recent studies reveal that even state-of-the-art pre-trained code models struggle with suggesting the correct APIs during code generation. However, the reasons for such poor API usage performance are barely investigated. To address this challenge, we propose using knowledge probing as a means of interpreting code models, which uses cloze-style tests to measure the knowledge stored in models. Our comprehensive study examines a code model's capability of understanding API fully qualified names from two different perspectives: API call and API import. Specifically, we reveal that current code models struggle with understanding API names, with pre-training strategies significantly affecting the quality of API name learning. We demonstrate that natural language context can assist code models in locating Python API names and generalize Python API name knowledge to unseen data. Our findings provide insights into the limitations and capabilities of current pre-trained code models, and suggest that incorporating API structure into the pre-training process can improve automated API usage and code representations. This work provides significance for advancing code intelligence practices and direction for future studies. All experiment results, data and source code used in this work are available at \url{https://doi.org/10.5281/zenodo.7902072}.

==> tab/_rq2.tex <==
\subsection{RQ2: Evaluation of API structural knowledge}
\begin{table*}[t]
    \centering
    % \resizebox{\columnwidth}{
    \begin{tabular}{ccc|cc| cc| cc| cc| cc| cc| cc}
     & & &\multicolumn{2}{c|}{$P@1$} & \multicolumn{2}{c|}{$P@5$} & \multicolumn{2}{c|}{$P@10$} & \multicolumn{2}{c}{$P@20$} & \multicolumn{2}{c}{$P@30$} & \multicolumn{2}{c}{$P@40$} & \multicolumn{2}{c}{$P@50$}\\
   & & & \multicolumn{1}{c}{S} & \multicolumn{1}{c|}{F} 
     & \multicolumn{1}{c}{S} & \multicolumn{1}{c|}{F} 
     & \multicolumn{1}{c}{S} & \multicolumn{1}{c|}{F} 
     & \multicolumn{1}{c}{S} & \multicolumn{1}{c|}{F} 
      & \multicolumn{1}{c}{S} & \multicolumn{1}{c|}{F} 
      & \multicolumn{1}{c}{S} & \multicolumn{1}{c|}{F} 
      & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{F} 
     \\\hline
    
    \multirow{4}{15mm}{CodeBERT\\-base-MLM} 
    & \multirow{2}{*}{F}
    & Mi.
    & 24.89& 10.28
    & 43.47& 25.24
    & 50.39& 33.82
    & 57.78& 42.01
    & 61.67& 46.75
    & 64.67& 49.76
    & 67.03& 52.32
    \\
    && Ma.
    & 24.61& 8.54
    & 44.01& 21.07
    & 51.23& 28.57
    & 58.89& 35.94
    & 62.81& 40.43
    & 65.90& 43.21
    & 68.20& 45.80
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 23.29& 10.28
    & 41.39& 25.24
    & 48.18& 33.82
    & 56.04& 42.01
    & 60.61& 46.75
    & 63.86& 49.76
    & 66.46& 52.32
    \\
    && Ma.
    & 20.24& 8.54
    & 37.31& 21.07
    & 44.21& 28.57
    & 52.22& 35.94
    & 57.03& 40.43
    & 60.49& 43.21
    & 63.18& 45.80
    \\\hline
    \multirow{4}{15mm}{CodeBERT-python}
    & \multirow{2}{*}{F}
   & Mi.
   & 30.46& 20.61
& 49.67& 37.35
& 58.23& 46.19
& 65.92& 55.11
& 70.44& 60.58
& 73.56& 64.30
& 75.80& 67.05
    \\
    && Ma.
    & 30.69& 17.23
& 51.31& 31.95
& 60.01& 40.05
& 67.61& 48.51
& 71.99& 53.93
& 74.99& 57.67
& 77.18& 60.59
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 25.55& 20.61
& 43.81& 37.35
& 51.53& 46.19
& 59.41& 55.11
& 63.91& 60.58
& 67.24& 64.30
& 70.03& 67.05
    \\
    && Ma.
    & 21.04& 17.23
& 39.39& 31.95
& 47.63& 40.05
& 55.86& 48.51
& 60.55& 53.93
& 64.12& 57.67
& 67.18& 60.59
    \\\hline\hline\hline
    \multirow{4}{15mm}{Graph\\CodeBERT-base}
    & \multirow{2}{*}{F}
   & Mi.
   & 27.18& 11.52
& 46.79& 25.55
& 54.32& 32.83
& 61.00& 40.47
& 64.84& 45.05
& 67.66& 48.76
& 70.09& 51.50
    \\
    && Ma.
    & 25.07& 9.52
& 45.66& 21.77
& 53.53& 28.32
& 60.46& 35.24
& 64.49& 39.61
& 67.23& 43.14
& 69.62& 45.79
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 26.86& 11.52
& 45.23& 25.55
& 51.99& 32.83
& 59.40& 40.47
& 64.17& 45.05
& 67.30& 48.76
& 69.58& 51.50
    \\
    && Ma.
    & 23.61& 9.52
& 41.09& 21.77
& 47.93& 28.32
& 55.47& 35.24
& 60.19& 39.61
& 63.52& 43.14
& 66.03& 45.79
    \\\hline\hline\hline
    \multirow{4}{15mm}{PLBART\\-base} 
    & \multirow{2}{*}{F}
   & Mi.
   & 1.88& 5.50
& 9.48& 15.12
& 15.05& 21.16
& 22.58& 28.38
& 27.81& 33.33
& 31.63& 37.20
& 34.88& 40.39
    \\
    && Ma.
    & 1.94& 4.95
& 9.93& 13.98
& 16.23& 19.31
& 24.56& 25.93
& 30.13& 30.37
& 34.04& 33.81
& 37.37& 36.71
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 0.43& 5.50
& 3.43& 15.12
& 7.10& 21.16
& 12.54& 28.38
& 15.77& 33.33
& 18.70& 37.20
& 21.13& 40.39
    \\
    && Ma.
    & 0.39& 4.95
& 3.00& 13.98
& 6.41& 19.31
& 11.30& 25.93
& 14.31& 30.37
& 17.28& 33.81
& 19.65& 36.71
    \\\hline
    \multirow{4}{15mm}{PLBART\\-large}
    & \multirow{2}{*}{F}
   & Mi.
   & 4.05& 7.22
& 13.11& 16.36
& 18.59& 21.89
& 24.56& 27.98
& 28.75& 31.75
& 32.15& 34.84
& 34.83& 37.46
    \\
    && Ma.
    & 4.31& 6.47
& 14.66& 14.99
& 20.83& 20.06
& 27.75& 25.90
& 32.35& 29.55
& 36.09& 32.35
& 38.84& 34.82
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 0.99& 7.22
& 5.20& 16.36
& 8.73& 21.89
& 13.15& 27.98
& 16.74& 31.75
& 19.69& 34.84
& 22.37& 37.46
    \\
    && Ma.
    & 0.89& 6.47
& 4.65& 14.99
& 7.99& 20.06
& 12.45& 25.90
& 16.04& 29.55
& 19.01& 32.35
& 21.69& 34.82
    \\\hline
    \multirow{4}{15mm}{PLBART\\-csnet} 
    & \multirow{2}{*}{F}
   & Mi.
   & 0.89& 1.61
& 4.85& 8.20
& 8.17& 12.20
& 12.86& 17.15
& 16.75& 20.46
& 20.10& 23.13
& 22.87& 25.32
    \\
    && Ma.
    & 0.71& 1.48
& 4.78& 7.28
& 8.33& 11.03
& 13.32& 15.51
& 17.39& 18.52
& 20.96& 21.09
& 23.87& 23.27
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 5.26& 1.61
& 18.47& 8.20
& 25.43& 12.20
& 33.14& 17.15
& 37.97& 20.46
& 41.47& 23.13
& 44.42& 25.32
    \\
    && Ma.
    & 4.61& 1.48
& 16.87& 7.28
& 23.47& 11.03
& 30.85& 15.51
& 35.82& 18.52
& 39.42& 21.09
& 42.37& 23.27
    \\\hline\hline
    \multirow{4}{15mm}{PLBART\\-Sum}
    & \multirow{2}{*}{F}
   & Mi.
   & 0.27& 2.46
& 3.94& 9.26
& 8.32& 13.95
& 13.65& 20.11
& 16.76& 24.32
& 19.45& 27.66
& 21.72& 30.36
    \\
    && Ma.
    & 0.23& 2.09
& 3.59& 8.05
& 7.55& 12.03
& 13.16& 17.59
& 16.37& 21.36
& 19.05& 24.23
& 21.54& 26.76
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 3.93& 2.46
& 12.33& 9.26
& 16.28& 13.95
& 21.23& 20.11
& 24.73& 24.32
& 27.65& 27.66
& 30.09& 30.36
    \\
    && Ma.
    & 3.48& 2.09
& 11.08& 8.05
& 14.97& 12.03
& 19.99& 17.59
& 23.53& 21.36
& 26.54& 24.23
& 29.15& 26.76
    \\\hline
    \multirow{4}{15mm}{PLBART\\-Gen}
    & \multirow{2}{*}{F}
   & Mi.
   & 1.69& 2.52
& 8.43& 12.51
& 13.35& 18.61
& 19.76& 25.43
& 23.69& 29.54
& 26.41& 32.69
& 28.60& 35.27
    \\
    && Ma.
    & 1.68& 2.49
& 9.01& 12.17
& 14.28& 18.18
& 21.45& 24.92
& 26.11& 29.04
& 29.05& 32.36
& 31.37& 34.97
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 5.32& 2.52
& 18.02& 12.51
& 25.31& 18.61
& 33.14& 25.43
& 38.07& 29.54
& 41.68& 32.69
& 44.48& 35.27
    \\
    && Ma.
    & 4.67& 2.49
& 16.74& 12.17
& 24.00& 18.18
& 32.03& 24.92
& 37.07& 29.04
& 40.86& 32.36
& 43.84& 34.97
    \\\hline
    \multirow{4}{15mm}{PLBART\\-MT}
    & \multirow{2}{*}{F}
   & Mi.
   & 1.75& 3.59
& 8.44& 13.23
& 13.98& 20.41
& 20.43& 28.72
& 24.33& 33.51
& 27.33& 37.08
& 29.61& 39.70
    \\
    && Ma.
    & 1.79& 3.29
& 8.29& 12.42
& 14.24& 19.08
& 21.45& 26.83
& 25.73& 31.51
& 29.10& 34.79
& 31.73& 37.36
    \\\cdashline{2-17}
    & \multirow{2}{*}{L}
    & Mi.
    & 7.00& 3.59
& 19.73& 13.23
& 27.13& 20.41
& 34.77& 28.72
& 39.65& 33.51
& 43.17& 37.08
& 45.84& 39.70
    \\
    && Ma.
    & 6.58& 3.29
& 18.74& 12.42
& 26.16& 19.08
& 34.12& 26.83
& 39.26& 31.51
& 42.86& 34.79
& 45.46& 37.36
    \\\hline
    \end{tabular}
    % }
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

==> tab/rq3_example.tex <==
\begin{table*}  []
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllll}\hline
        & \textbf{Test} & \textbf{Answer} &\textbf{NL Context}  & \textbf{PLBART-Large}\\\hline
        & \multirow{2}{*}{numpy.random.\underline{\hspace{0.5cm}}\_normal}
        &\multirow{2}{*}{standard}
        & 
        
        &normal [0.10], \_ [0.06], RandomState [0.06], randn [0.06], rand [0.06]\\
        && &The fill function.&\_ [0.63], normal [0.05], random [0.02], Random [0.02], \textbf{standard [0.02]}, rand [0.01]
        \\\hdashline
       &
       & 
       & 
       & 
       \\&&&&
       \\\hdashline
        &\multirow{2}{*}{from scipy.ndimage.interpol\underline{\hspace{0.5cm}} import affine\_transform}
       &  \multirow{2}{*}{ation}
       & 
       
       & import [0.99], . [0.00], to [0.00], ( [0.00], from [0.00]
       \\&&&do random rotation&import [1.00], . [0.00], \textbf{ation [0.00]}, ations [0.00], ... [0.00]
       \\\hdashline
       &\multirow{2}{*}{from numpy.\underline{\hspace{0.5cm}} import decode}
       &  \multirow{2}{*}{char}
       & 
       
       & from [0.25], core [0.17], import [0.09], lib [0.05], \textbf{char [0.04]}
       \\&&&add cf from wrfioapi&from [0.32], lib [0.09], core [0.07], \textbf{char [0.05]}, </s> [0.03]
       \\\hdashline
       & \multirow{2}{*}{from \underline{\hspace{0.5cm}}.modules import update}
       &\multirow{2}{*}{\textcolor{gray}{Ġ}sys}
       & 
       
       &\textcolor{gray}{Ġ}django [0.12], \textcolor{gray}{Ġ}twisted [0.06], \textcolor{gray}{Ġ}calib [0.04], . [0.03], \textcolor{gray}{Ġ}nltk [0.03]
       \\&&&Adds a list of modules to sys.modules.&\textbf{\textcolor{gray}{Ġ}sys [0.16]}, . [0.15], \textcolor{gray}{Ġ}django [0.08], \_\_ [0.06], \textcolor{gray}{Ġ}os [0.04]
       \\\hdashline
       & \multirow{2}{*}{from os import \underline{\hspace{0.5cm}}cwdu}
       &\multirow{2}{*}{\textcolor{gray}{Ġ}get}
       & 
       
       & \textcolor{gray}{Ġ}path [0.28], \textcolor{gray}{Ġ}stat [0.07], \textcolor{gray}{Ġ}listdir [0.05], \textcolor{gray}{Ġ}popen [0.05], \textcolor{gray}{Ġ}chmod [0.05]
       \\&&&Return a relative version of a path&\textcolor{gray}{Ġ}path [0.66], \textcolor{gray}{Ġ}getcwd [0.04], \textcolor{gray}{Ġ}sep [0.03], \textcolor{gray}{Ġ}system [0.02], \textbf{\textcolor{gray}{Ġ}get [0.02]}
    \\\hline
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

==> tab/rq4_example.tex <==
\begin{table*} []
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llll}\hline
    \textbf{}&\textbf{Test} &\textbf{Answer} &\textbf{GraphCodeBERT-MLM}\\\hline
    \multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Seen}}}
        & django.\underline{\hspace{0.5cm}}.settings.NOTIFICATION\_LANGUAGE\_MODULE
        &conf
        & \textbf{conf [0.30]}, core [0.19], app [0.90], foundation [0.08], admin [0.08]\\
        & \underline{\hspace{0.5cm}}p8radius.radius.Radius.from\_diff
        & \textcolor{gray}{Ġ}pe
        & \textbf{\textcolor{gray}{Ġ}pe [0.97]}, \textcolor{gray}{Ġ}open [0.01], \# [0.00], \textcolor{gray}{Ġ}j [0.00], \textcolor{gray}{Ġ}< [0.00]\\
       &from logging.\underline{\hspace{0.5cm}}ger import info
       &Log
       &  log [0.94], \textcolor{gray}{Ġ}Log [0.06], \textbf{Log [0.00]}, bad [0.00], debug [0.00]\\
       &from mimicdb.\underline{\hspace{0.5cm}}end import sismember
       &back
       & \textbf{back [0.99]}, ext [0.00], front [0.00], z [0.00], \textcolor{gray}{Ġ}back [0.00]\\
       &from PIL.\underline{\hspace{0.5cm}}.open import resize
       &Image
       &\textbf{Image [0.71]}, image [0.08], Core [0.04], Images [0.03], util [0.02]\\
       &from wx.Text\underline{\hspace{0.5cm}} import GetValue
       &Ctrl
       &\textbf{Ctrl [0.56]}, Field [0.08], Area [0.06], Input [0.03], IO [0.02]\\
       &from redis.from\_\underline{\hspace{0.5cm}} import set
       &url
       &set [0.39], list [0.09], queue [0.09], modules [0.08], pool [0.05]
       \\\hline\hline
       \multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Seen}}}
       &saga.filesystem.File.\underline{\hspace{0.5cm}}
       &copy
       &File [0.11], write [0.04], create [0.03], get [0.03], file [0.02]
       \\
       &lxml.objectify.\underline{\hspace{0.5cm}}parser
       &make
       &xml [0.44], DOM [0.07], Sub [0.05], ML [0.05], sub [0.04]
       \\
       
        &from tensorflow.\underline{\hspace{0.5cm}} import conj
        &math
        &base [0.19], core [0.13], comp [0.10], types [0.04], node [0.03]
        \\
        &from dddp.\underline{\hspace{0.5cm}}.API import do\_unsub
        &api
        &\textbf{api [0.15]}, core [0.09], client [0.06], API [0.05], base [0.04]
        \\
        &from meshlab\underline{\hspace{0.5cm}}.transform import vert\_function
        &xml
        &els [0.46], plot [0.09], js [0.07], la [0.02], ui [0.01]
        \\
        &from \underline{\hspace{0.5cm}}oto3.session.Session import resource
        & \textcolor{gray}{Ġ}b
        & \textbf{\textcolor{gray}{Ġ}b [1.00]}, \textcolor{gray}{Ġ}rob [0.00], \textcolor{gray}{Ġ}B [0.00], b [0.00], \textcolor{gray}{Ġ}m [0.00]
        \\
        &from ipywidgets import \underline{\hspace{0.5cm}}Box
        &\textcolor{gray}{Ġ}H, \textcolor{gray}{Ġ}V
        &\textbf{\textcolor{gray}{Ġ}V [0.16]}, \textcolor{gray}{Ġ}Q [0.15], \textcolor{gray}{Ġ}Combo [0.10], \textbf{\textcolor{gray}{Ġ}H [0.10]}, \textcolor{gray}{Ġ}List [0.08]
        \\\hline
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
